Box for Mask and Mask for Box: weak losses for multi-task partially supervised learning

Object detection and semantic segmentation are both scene understanding tasks yet they differ in data structure and information level. Object detection requires box coordinates for object instances while semantic segmentation requires pixel-wise class labels. Making use of one task's information to train the other would be beneficial for multi-task partially supervised learning where each training example is annotated only for a single task, having the potential to expand training sets with different-task datasets. This paper studies various weak losses for partially annotated data in combination with existing supervised losses. We propose Box-for-Mask and Mask-for-Box strategies, and their combination BoMBo, to distil necessary information from one task annotations to train the other. Ablation studies and experimental results on VOC and COCO datasets show favorable results for the proposed idea. Source code and data splits can be found at https://github.com/lhoangan/multas.

==> Sections/slide0_intro.tex <==
\section[Intro]{Introduction}


\begin{frame}{Motivation (1/3)}

    Object detection and semantic segmentation:

    \begin{figure}
        \centering
        \includegraphics[width=.36\textwidth]{Images/bus.png}
        \includegraphics[width=.37\textwidth]{Images/motorbike.png}
        \label{fig:det_seg}
    \end{figure}

    \pause

    image understanding
    \begin{columns}
        \begin{column}{.5\textwidth}
            \begin{itemize}
                \item Object detection
                \begin{itemize}
                    \item instance object level
                    \item regressing localization
                    \item concrete objects only
                \end{itemize}
            \end{itemize}
        \end{column}
        \begin{column}{.5\textwidth}
            \begin{itemize}
                \item Semantic segmentation
                \begin{itemize}
                    \item category level
                    \item per-pixel prediction
                    \item amorphous regions
                \end{itemize}
            \end{itemize}
        \end{column}
    \end{columns}
    
    \note{
        To begin with, let's talk about  OD and SS.
        Obviously, everybody knows about
        Both aim to understand image contents.
        different in spatial structure and information granularity.
        \begin{itemize}
            \item object detection distinguishes different object instances,
            semantic segmentation recognizes category and amorphous regions
        \end{itemize}
    }
\end{frame}


\begin{frame}{Motivation (2/2)}
    Multi-task learning
    \begin{itemize}
        \item assumes inherently related tasks
        \item requires feature compatibility
        \item includes shared encoder + separated heads for each task
    \end{itemize}

    \note{
        Instead of combining the 2 tasks, we want to learn them as they are

        using a multi-task learning framework

        so by jointly optimizing both tasks for each training example, we can
        learn salient interrelationship.

        in this paper, we approach the problem in a little different way
    }

    \pause

    Partially annotated data: each image is annotated with only 1 task
    \begin{itemize}
        \item hinders jointly learning shared representation per image
        \item data efficient, more training data from various sources
    \end{itemize}

    \note{
        can use different datasets with different task annotations to improve
        training
    }

\end{frame}

\begin{frame}{Multi-task partially supervised learning}

    \begin{figure}[t]
        \centering
        \small
        \def\svgwidth{\textwidth}
        \input{Images/MTL_general_A.pdf_tex}
    \end{figure}
    
\end{frame}

\begin{frame}{Objectives}

    Box-for Mask and Mask-for-Box training

    \begin{figure}[t]
        \centering
        \footnotesize
        \def\svgwidth{\textwidth}
        \input{Images/MTL_general_B.pdf_tex}
    \end{figure}

\end{frame}


==> Sections/slide1_method.tex <==
\section[Method]{Method}

\begin{frame}{Multi-task Partially Supervised Learning}


    \only<1>{
        
        \begin{figure}[t]
            \centering
            \scriptsize
            \def\svgwidth{.8\textwidth}
            \input{Images/MTL_general_A.pdf_tex}
        \end{figure}
    
        $$
            \label{eq:loss}
            \mathcal{L} =            \mathcal{L}_\text{det} 
                            + \lambda\mathcal{L}_\text{seg} 
        $$
    }
    
    \only<2>{
    
        \begin{figure}[t]
            \centering
            \scriptsize
            \def\svgwidth{.8\textwidth}
            \input{Images/MTL_general_B.pdf_tex}
        \end{figure}
    
        $$
            \label{eq:loss}
            \mathcal{L} =            \left(\mathcal{L}_\text{det} + \mathcal{L}_\text{M4B}\right)
                            + \lambda\left(\mathcal{L}_\text{seg} + \mathcal{L}_\text{B4M}\right)
        $$
    }

    
\end{frame}

\begin{frame}{Mask-for-Box learning}

    \hbox{
        \hspace{-3.3em}
        \def\svgwidth{1.16\textwidth}
        \tiny
        \input{Images/MTL_M4B.pdf_tex}
    }

    Observation: semantic masks can produce bounding boxes
    \begin{itemize}
        \item (1) used as-is \inlinegraphics{add} (2) split \inlinegraphics{split} (3) merged with the others \inlinegraphics{merge}
        \item predicted boxes contain objectness information
    \end{itemize}
\end{frame}

\begin{frame}{Mask-for-Box visualization}

\begin{figure}[t]
    \centering
    \includegraphics[width=.83\linewidth]{Images/m4b_illust/1_feh_2757020_000003_epoch-46.png} %
    \includegraphics[width=.83\linewidth]{Images/m4b_illust/1_feh_2757020_000027_epoch-30.png} %
    \includegraphics[width=.83\linewidth]{Images/m4b_illust/2_feh_2757020_000009_epoch-56.png} %
    \includegraphics[width=.83\linewidth]{Images/m4b_illust/0_feh_2757020_000013_epoch-23.png} %
    \label{fig:qualitative1}
\end{figure}

    
\end{frame}

\begin{frame}{Box-for-Mask learning}

    \hbox{
        \hspace{-3.2em}
        \def\svgwidth{1.16\textwidth}
        \tiny
        \only<1>{\input{Images/MTL_B4M_stage1.pdf_tex}}
        \only<2>{\input{Images/MTL_B4M_stage2.pdf_tex}}
        \only<3>{\input{Images/MTL_B4M.pdf_tex}}
    }

    $$
        \mathcal{L}_\text{B4M} = \mathcal{L}_\text{CE}\left(M, M^c\right)
        \uncover<2-3>{+ \mathcal{L}_{L2}\left(\alpha, M^b\right)}
        \uncover<3>{  + \mathcal{L}_{\text{object}}}
    $$

    \uncover<3>{
        $$ \mathcal{L}_{\text{object}} = \sum_{k=0}^{n_B}\max\left(0, \gamma +
            d_\mathbb{E}\left(\bar{\mathbf{z}}_k, \bar{\mathbf{z}}_k^+\right) -
            d_\mathbb{E}\left(\bar{\mathbf{z}}_k, \bar{\mathbf{z}}_k^-\right)\right),
        $$
    }

 
\end{frame}


==> Sections/slide2_experiments.tex <==
\section{Experiments}

\begin{frame}{Dataset}

    Pascal VOC + augmented VOC: 20 categories

    Simulating multi-task scenario:
    \begin{itemize}
        \item detection subset \protect\hleft\ (7,558 images)
        \item segmentation subset \protect\hright\  (7,656 images)
    \end{itemize}

    \note{
        To simulate the partial supervision scenario,

        images are randomly sampled into 2 subsets,

        detection whose semantic annotations are held back and

        the other for semantic segmentation whose bounding-box annotations are kept out.
    }
    
\end{frame}

\begin{frame}{M4B: Training for Boxes \only<2>{ | TIDE analysis} \only<3>{ | SOTA comparison}}

    \only<1>{\input{Tables/Table1_M4B}}
    
    \only<2>{\includegraphics[width=\textwidth]{Images/TIDE_vis.png}}
    \scalebox{.85}{\begin{minipage}{\textwidth}
        \only<2>{\input{Tables/Table1_TIDE}}
        \end{minipage}
    }
    \scalebox{.85}{\begin{minipage}{\textwidth}
        \only<3>{\input{Tables/Table1_SOTA}}
        \end{minipage}
    }

    \note{
        \only<2>{
            
        
        }
    }
    
\end{frame}

\begin{frame}{B4M: Training for Masks}

    \input{Tables/Table2}
    
\end{frame}

\begin{frame}{BoMBo: comparing to SOTA}

    \scalebox{.85}{\begin{minipage}{\textwidth}
        \input{Tables/Table3}
    \end{minipage}
    }
    
\end{frame}

\begin{frame}{Discussion}
    Partially annotated data: no images with both task annotations.

    \begin{itemize}
        \item alternating training between 2 tasks
        \item multi-task setting shows favorable results
        \item out-of-domain multi-task remains an unexplored problem.
    \end{itemize}
\end{frame}


==> Tables/Table2_poster.tex <==
\begin{table}[t]
  \centering
  \begin{tabular}{@{}llcccc@{}}
     \toprule
                                                      &         & ResNet18 & ResNet50  &   SwinT  &   SwinB  \\ %
     \midrule
     \color[HTML]{008000}$\lambda\mathcal{L}_\text{seg}$&\hleft   &   65.292 &    69.065 &   75.012 &   79.690 \\% vyr9u51c & r1y9qll5 & 1rqn98gk & 2il4g0q2 
     $\; \color[HTML]{0000ff}+ \mathcal{L}_\text{CE}$   &\pie{360}&   64.740 &    67.582 &   73.830 &   78.510 \\% 2a3ir6cv & 6p7zfv1o & 2x2kjn8w & 1gfwbq2w 
     $\;\quad \color[HTML]{0000ff}+\mathcal{L}_\text{L2}$                    &\pie{360}&   67.623 &    71.763 &   76.269 &   80.654 \\% yylt9mg0 & 2lsl091y & 2j8p98nd & 14azj4f6 
     $\qquad+$ B2S Affinity~\cite{Kulharia2020Box2Seg}  &\pie{360}&   66.954 &    71.562 &   76.266 &   80.880 \\% 338dwyzx & sbpt19g5 & 1vywks9x& 30d3ofz6 
     $\qquad+$ Shifting Rate~\cite{Song2023BCM}         &\pie{360}&   67.325 &    71.164 &   76.657 &\bf81.264 \\% 2oc1jwbs & 1ou8sp5v & 177uwrzv& 3eaucicq 
     $\qquad\color[HTML]{0000ff}+ \mathcal{L}_\text{triplet}$&\pie{360}&\bf68.545 &\bf 72.306 &\bf76.981 &   81.236 \\% gsux9keh & 1ugm7zp6 & 2gt4gbvc & 20hj02z9 
     \bottomrule
  \end{tabular}
  \caption{Performance of B4M losses when training box-annotated with supervised images (baseline).
  Simply applying cross-entropy loss ($\mathcal{L}_S$) on pseudo-masks (without attention maps)
  produces negative effects %
  but adding the attention loss ($\mathcal{L}_\alpha$) provides a boost. The triplet object
  loss ($\mathcal{L}_\text{object}$) is generally more helpful than the other approaches.
  }
  \label{tab:B4M}
\end{table}


==> colors.tex <==
\definecolor{CanvasBG}{HTML}{FAFAFA}

\definecolor{UnccGreen}{HTML}{00703C}
\definecolor{UnccGold}{HTML}{B3A369}
\definecolor{UnccLightGreen}{HTML}{C3D7A4}
\definecolor{UnccYellow}{HTML}{F0CB00}
\definecolor{UnccOrange}{HTML}{F3901D}
\definecolor{UnccLightYellow}{HTML}{FFF6DC}
\definecolor{UnccBlue}{HTML}{00728F}
\definecolor{UnccPink}{HTML}{DE3A6E}
\definecolor{White}{HTML}{FFFFFF}
\definecolor{LightGray}{HTML}{DDDDDD}

\definecolor{WarmGray}{HTML}{696158}
\definecolor{StoneGray}{HTML}{717C7D}
\definecolor{DarkGreen}{HTML}{2C5234}
\definecolor{LightGreen}{HTML}{509E2F}
\definecolor{BrightGold}{HTML}{F0CB00}

\definecolor{Royal}{HTML}{72246C}
\definecolor{Ocean}{HTML}{006BA6}
\definecolor{Flash}{HTML}{B52555}
\definecolor{Citrus}{HTML}{FFB81C}
\definecolor{Spring}{HTML}{CEDC00}

\definecolor{Garden}{HTML}{B7CE95}
\definecolor{Sand}{HTML}{F0E991}
\definecolor{Bloom}{HTML}{F1E6B2}
\definecolor{Clay}{HTML}{B7B09C}
\definecolor{Cloud}{HTML}{BAC5B9}


\definecolor{header}{HTML}{AFBBE1}%
\definecolor{maroon}{HTML}{800000}
\definecolor{greenDark}{HTML}{00712D}
\definecolor{frame_bg}{HTML}{FFF1DB}
\definecolor{blueDark}{HTML}{667BC6}%

\setbeamercolor{frametitle}{bg=maroon}
\setbeamercolor{progress bar}{bg=Garden, fg=maroon}
\setbeamercolor{alerted text}{fg=Flash}

\setbeamercolor{block title}{bg=LightBlue, fg=White}
\setbeamercolor{block title example}{bg=Ocean, fg=White}
\setbeamercolor{block title alerted}{bg=header, fg=White}
\setbeamercolor{block body}{bg=CanvasBG}

\metroset{titleformat=smallcaps, progressbar=foot}

\makeatletter
\setlength{\metropolis@progressinheadfoot@linewidth}{2pt}
\setlength{\metropolis@titleseparator@linewidth}{2pt}
\setlength{\metropolis@progressonsectionpage@linewidth}{2pt}

